On Privacy Weaknesses and Vulnerabilities in Software Systems

In this digital era, our privacy is under constant threat as our personal data and traceable online/offline activities are frequently collected, processed and transferred by many software applications. Privacy attacks are often formed by exploiting vulnerabilities found in those software applications. The Common Weakness Enumeration (CWE) and Common Vulnerabilities and Exposures (CVE) systems are currently the main sources that software engineers rely on for understanding and preventing publicly disclosed software vulnerabilities. However, our study on all 922 weaknesses in the CWE and 156,537 vulnerabilities registered in the CVE to date has found a very small coverage of privacy-related vulnerabilities in both systems, only 4.45\% in CWE and 0.1\% in CVE. These also cover only a small number of areas of privacy threats that have been raised in existing privacy software engineering research, privacy regulations and frameworks, and relevant reputable organisations. The actionable insights generated from our study led to the introduction of 11 new common privacy weaknesses to supplement the CWE system, making it become a source for both security and privacy vulnerabilities.

==> sections/tbl-individual-rights.tex <==
\begin{table}
\caption{Individual rights on privacy}
\label{tab:rights}
\begin{tabular}{p{3.75cm} p{3.75cm}}
	\toprule
	Rights &
	Relevant data protection regulations/privacy acts \\ \midrule
	Right to be informed &
	GDPR, CCPA, HIPAA, GLBA, APA \\
	Right of access &
	GDPR, HIPAA, USPA, APA \\
	Right to rectification &
	GDPR, HIPAA, USPA, APA \\
	Right to erasure &
	GDPR, CCPA \\
	Right to restrict of processing &
	GDPR, HIPAA \\
	Right to data portability &
	GDPR \\
	Right to object &
	GDPR, APA \\
	Right in relation to automated decision making and profiling &
	GDPR \\
	Right to opt-out of sale &
	CCPA \\
	Right to non-discrimination &
	CCPA \\
	Right to request confidential communications &
	HIPAA \\
	Right to be protected against unwarranted invasion &
	GDPR, USPA \\
	Right to make a complaint &
	GDPR, APA \\
	Right to opt-out of sharing &
	GLBA \\
	Right to not identifying yourself &
	APA \\ \bottomrule
\end{tabular} 
\footnotesize \flushleft{\textit{GDPR: European General Data Protection Regulations, CCPA: California Consumer Privacy Act, HIPAA: Health Insurance Portability and Accountability Act, USPA, U.S. Privacy Act, GLBA: Gramm-Leach Bliley Act and APA: Australian Privacy Act.}}
\end{table}

\begin{comment}
\begin{table*}[ht]
\caption{Individual rights on privacy}
\label{tab:rights}
\begin{tabular}{p{4cm} p{10cm} p{3cm}}
\toprule
Rights &
  Description &
  Relevant data protection regulations/privacy acts \\ \midrule
Right to be informed &
  Individuals must be informed about the collection, use and processing of their personal data. For example, the software applications must inform the purposes of personal data collection and processing. In case the personal data is processed by other parties, the individuals must be informed to whom their personal data is disclosed/transferred. &
  GDPR, CCPA, HIPAA, GLBA, APA \\
Right of access &
  Individuals must be able to request to access and receive a copy of their personal data. &
  GDPR, HIPAA, USPA, APA \\
Right to rectification &
  Individuals must be able to request to correct, complete and/or make changes to their personal data. &
  GDPR, HIPAA, USPA, APA \\
Right to erasure &
  Individuals must be able to request to erase their personal data. &
  GDPR, CCPA \\
Right to restrict of processing &
  Individuals must be able to request to restrict of personal data processing. &
  GDPR, HIPAA \\
Right to data portability &
  Individuals must be able to request obtain, reuse, move, copy or transfer their personal data across different services for their own purposes. &
  GDPR \\
Right to object &
  Individuals must be able to object to the processing of their personal data in certain circumstances (e.g. direct marketing). &
  GDPR, APA \\
Rights in relation to automated decision making and profiling &
  Organisations must obtain consent from individuals when the software may process their personal data based on automated decision making and profiling. &
  GDPR \\
Right to opt-out of sale &
  Individuals must be able to request to opt-out if their personal data is sold by organisations. &
  CCPA \\
Right to non-discrimination &
  Individuals, who exercise their individual rights with respect to particular regulations, must be provided with the same quality and price of goods and services by businesses. &
  CCPA \\
Right to request confidential communications &
  Individuals must be able to request to change means or location for receiving communication of health information. &
  HIPAA \\
Right to be protected against unwarranted invasion &
  Personal data must be protected from invasion resulting from the collection, use, disclosure, maintenance and other processing. &
  GDPR, USPA \\
Right to make a complaint &
  Individuals must be able to lodge a complaint to relevant organisations or supervisory authority if their personal data is mishandled. &
  GDPR, APA \\
Right to opt-out of sharing &
  Individuals must be able to opt-out from sharing their personal data. &
  GLBA \\
Right to not identifying yourself &
  Individuals must have an option not identifying themselves in certain circumstances (e.g. using pseudonym). &
  APA \\ \bottomrule
\end{tabular}
\vspace{0.5mm}
\\
\footnotesize \flushleft{\textit{GDPR: European General Data Protection Regulations, CCPA: California Consumer Privacy Act, HIPAA: Health Insurance Portability and Accountability Act, USPA, U.S. Privacy Act, GLBA: Gramm-Leach Bliley Act and APA: Australian Privacy Act.}}
\end{table*} 
\end{comment}

==> sections/tbl-venues.tex <==
\begin{table*}[h]
	\caption{Selected software engineering publication venues.}
	\label{tab:venues}
	\begin{tabular}{p{8.5cm} p{1.25cm} p{1.5cm} p{1cm} p{1.25cm} p{1.25cm}}
		\toprule \textbf{Source title} & \textbf{Acronym} & \textbf{Type} & \textbf{Count} & \textbf{Included} & \textbf{Threats found} \\ \midrule
		ACM Transactions on Software Engineering and Methodology & TOSEM & Journal & 4 & 1 & 0\\
		Empirical Software Engineering & EMSE & Journal & 6 & 3 & 0\\
		IEEE Symposium on Security and Privacy & S\&P & Symposium & 330 & 64 & 9\\
		IEEE Symposium on Security and Privacy Workshops & SPW & Workshop & 134 & 49 & 5\\
		IEEE Transactions on Software Engineering & TSE & Journal & 22 & 7 & 1\\
		Information and Software Technology & IST & Journal & 16 & 5 & 0\\
		International Conference on Automated Software Engineering & ASE & Conference & 20 & 8 & 3\\
		International Conference on Availability, Reliability and Security & ARES & Conference & 186 & 113 & 93\\
		International Conference on Foundations of Software Engineering & FSE & Conference & 13 & 5 & 0\\
		International Conference on Mining Software Repositories & MSR & Conference & 8 & 2 & 0\\
		International Conference on Software Engineering & ICSE & Conference & 90 & 22 & 4\\
		International Requirements Engineering Conference & RE & Conference & 68 & 25 & 2\\
		International Symposium on Empirical Software Engineering and Measurement & ESEM & Conference & 5 & 1 & 0\\
		International Workshop on Evolving Security and Privacy Requirements Engineering & ESPRE & Workshop & 32 & 7 & 0\\
		Requirements Engineering & REJ & Journal & 19 & 10 & 2\\
		Symposium on Usable Privacy and Security & SOUPS & Symposium & 104 & 77 & 47 \\
		Systems and Software & JSS & Journal & 377 & 18 & 13 \\			
		\midrule
		\textbf{Sum} & & & \textbf{1,434} & \textbf{417} & \textbf{179} \\ \bottomrule
	\end{tabular}
\end{table*}

